Demonstration-Guided Reinforcement Learning with Efficient Exploration for Task Automation of Surgical Robot

Task automation of surgical robot has the potentials to improve surgical efficiency. Recent reinforcement learning (RL) based approaches provide scalable solutions to surgical automation, but typically require extensive data collection to solve a task if no prior knowledge is given. This issue is known as the exploration challenge, which can be alleviated by providing expert demonstrations to an RL agent. Yet, how to make effective use of demonstration data to improve exploration efficiency still remains an open challenge. In this work, we introduce Demonstration-guided EXploration (DEX), an efficient reinforcement learning algorithm that aims to overcome the exploration problem with expert demonstrations for surgical automation. To effectively exploit demonstrations, our method estimates expert-like behaviors with higher values to facilitate productive interactions, and adopts non-parametric regression to enable such guidance at states unobserved in demonstration data. Extensive experiments on $10$ surgical manipulation tasks from SurRoL, a comprehensive surgical simulation platform, demonstrate significant improvements in the exploration efficiency and task success rates of our method. Moreover, we also deploy the learned policies to the da Vinci Research Kit (dVRK) platform to show the effectiveness on the real robot. Code is available at https://github.com/med-air/DEX.

==> table/main_rliable.tex <==

\begin{table*}[t]
%\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\caption{\textbf{Aggregate performance after training 100k environment steps.}
% Normalized scores of our \ourmethod and baselines over each task domain. 
It presents interquartile mean and 95\% bootstrap confidence intervals over 10 runs. Each run is averaged over 20 evaluations.
% The highest performing scores are bolded.
}\vspace{-1mm}
\label{tab:main_agg}
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l|cc|ccc|cc|c}
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Reinforcement Learning}} & \multicolumn{3}{c}{\textbf{Imitation Learning}} & \multicolumn{2}{c}{\textbf{Demonstration-guided RL}} & \multicolumn{1}{c}{\textbf{Ours}} \\
\toprule
\textbf{Domains} & \textbf{SAC} & \textbf{DDPG} & \textbf{BC} & \textbf{SQIL} & \textbf{VINN} & \textbf{Replay}  & \textbf{BC+RL} & \textbf{\ourmethod}  \\\midrule
PSM         & $0.00 \scriptstyle{(0.00,0.00)}$  & $0.00 \scriptstyle{(0.00,0.00)}$ & $0.40 \scriptstyle{(0.35,0.45)}$   & $0.00 \scriptstyle{(0.00,0.00)}$ & $0.02 \scriptstyle{(0.00,0.04)}$ & $0.78 \scriptstyle{(0.72,0.83)}$   & $0.80 \scriptstyle{(0.76,0.84)}$ & $\mathbf{0.89\scriptstyle{(0.86,0.92)}}$ \\
Bi-PSM     & $0.00 \scriptstyle{(0.00,0.00)}$  & $0.00 \scriptstyle{(0.00,0.00)}$ & $0.08 \scriptstyle{(0.04,0.11)}$ & $0.00 \scriptstyle{(0.00,0.00)}$ & $0.00 \scriptstyle{(0.00,0.00)}$ & $0.00 \scriptstyle{(0.00,0.00)}$  & $0.00 \scriptstyle{(0.00,0.00)}$ & $\mathbf{0.39 \scriptstyle{(0.28,0.50)}}$ \\
ECM        & $0.96 \scriptstyle{(0.90,1.00)}$  & $0.99 \scriptstyle{(0.97,1.00)}$ & $\mathbf{1.00 \scriptstyle{(1.00,1.00)}}$ & $0.24 \scriptstyle{(0.18,0.30)}$ & $0.58 \scriptstyle{(0.52,0.63)}$ & $\mathbf{1.00 \scriptstyle{(1.00,1.00)}}$  & $\mathbf{1.00 \scriptstyle{(1.00,1.00)}}$ & $\mathbf{1.00 \scriptstyle{(0.98,1.00)}}$ \\
\midrule
Overall    & $0.32 \scriptstyle{(0.29,0.33)}$ & $0.43 \scriptstyle{(0.42,0.44)}$  & $0.68 \scriptstyle{(0.66,0.69)}$ & $0.02 \scriptstyle{(0.00,0.03)}$ & $0.24 \scriptstyle{(0.22,0.27)}$ & $0.80 \scriptstyle{(0.76,0.85)}$  & $0.83 \scriptstyle{(0.81,0.86)}$ & $\mathbf{0.92 \scriptstyle{(0.90,0.93)}}$\\
\bottomrule
\end{tabular}
}
\vspace{-0.175in}
\end{table*}
